Approximate Differentiable Rendering with Algebraic Surfaces

Differentiable renderers provide a direct mathematical link between an object's 3D representation and images of that object. In this work, we develop an approximate differentiable renderer for a compact, interpretable representation, which we call Fuzzy Metaballs. Our approximate renderer focuses on rendering shapes via depth maps and silhouettes. It sacrifices fidelity for utility, producing fast runtimes and high-quality gradient information that can be used to solve vision tasks. Compared to mesh-based differentiable renderers, our method has forward passes that are 5x faster and backwards passes that are 30x faster. The depth maps and silhouette images generated by our method are smooth and defined everywhere. In our evaluation of differentiable renderers for pose estimation, we show that our method is the only one comparable to classic techniques. In shape from silhouette, our method performs well using only gradient descent and a per-pixel loss, without any surrogate losses or regularization. These reconstructions work well even on natural video sequences with segmentation artifacts. Project page: https://leonidk.github.io/fuzzy-metaballs

==> moose_data.tex <==
\begin{figure}
  \centering
   \includegraphics[width=0.95\linewidth]{moose/sfs_moose.jpg}
    \caption{\textbf{SFS reconstruction on natural images} from a handheld cell phone video, using COLMAP~\cite{schoenberger2016mvs} and Mask RCNN~\cite{He2017MaskR} for automatic camera poses and silhouettes. The low degree of freedom allows the system to naturally recover from small errors in camera poses and segmentation, such as the tip of the nose.  }
    \label{fig:moose}
\end{figure}

==> moose_recon.tex <==
\begin{figure}[tbh]
     \centering
     \begin{subfigure}[t]{0.23\linewidth}
         \centering
         \includegraphics[trim={2cm 0 2cm 0},clip,width=\linewidth]{rebut_fig/plane_pyt3d.jpg}
         \caption{\textbf{SoftRas Mesh} ShapeNet Airplane}
         \label{fig:pyt_plane}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.23\linewidth}
         \centering
         \includegraphics[trim={2cm 0 2cm 0},clip,width=\linewidth]{rebut_fig/yoga2_dss.jpg}
         \caption{\textbf{PyT3D Point Cloud} Figurine }
         \label{fig:dss_yoga}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.23\linewidth}
         \centering
         \includegraphics[trim={2cm 0 2cm 0},clip,width=\linewidth]{figures/plane_mine_when_nocb4.jpg}
         \caption{\textbf{FM (Ours)} ShapeNet Airplane}
         \label{fig:out_plane}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.23\linewidth}
         \centering
         \includegraphics[trim={2cm 0 2cm 0},clip,width=\linewidth]{figures/yoga_mine_eccv.jpg}
         \caption{\textbf{FM (Ours)} Yoga Figurine }
         \label{fig:out_yoga}
     \end{subfigure}
   \caption{\textbf{Qualitative baselines for shape-from-silhouette experiments} We used a ShapeNet airplane for the mesh baseline ~\cite{kato2017neural,liu2019soft,ravi2020pytorch3d} and the figurine of existing point cloud differentiable renderers~\cite{DSS_points}. Our best-effort mesh-based baseline result was incoherent and the point cloud baseline had spurious points. }
   \label{fig:rebutrecon}
\end{figure}

==> old_content.tex <==
\begin{table}[th!]
  \centering
\begin{tabular}{lccc|cc|c}
\toprule
            &  Depth &   Mask &  Params  & Avg $\epsilon_R$ & Avg $\epsilon_T$ &  Avg \\
\midrule
           Initalizations & \xmark & \xmark &        &              16. &             21.2 & 18.4 \\
\midrule

Pulsar ~\cite{lassner2020pulsar} & \xmark & \cmark &    1200 &               16. &             21.3 & 18.4 \\
Point Cloud ~\cite{ravi2020pytorch3d} & \xmark & \cmark &    1200 &               16. &             17.5 & 16.7 \\
SoftRas Mesh ~\cite{liu2019soft}& \xmark & \cmark &     750 &               15. &             10.0 & 12.1 \\
SoftRas Mesh ~\cite{liu2019soft}& \cmark & \cmark &     750 &                15. &             11.3 & 12.7 \\
 \midrule

Point-Point ICP  & \cmark & \xmark &    1200 &               3.2 &             3.23 & 2.87 \\
Point-Plane ICP & \cmark & \xmark &    1200 &              3.3 &             3.22 & 3.09 \\
Point-Point ICP & \cmark & \xmark &   120000 &             \textbf{2.1} &             2.44 & 2.11 \\
Point-Plane ICP & \cmark & \xmark &   120000 &              2.2 &             \textbf{2.24} & 1.96 \\
\midrule
Fuzzy Metaballs & \xmark & \cmark &     400 &               3.5 &             3.54 & 3.25 \\
Fuzzy Metaballs & \cmark & \cmark &     400 &               2.6 &             2.49 & \textbf{1.82} \\
\bottomrule
\end{tabular}
\caption{\textbf{Noise Free Pose Estimation} PyTorch3D~\cite{ravi2020pytorch3d} provides differentiable rendering baselines while Open3D~\cite{Zhou2018} provides point cloud ICP baselines. Errors are specified as the geometric mean of position (in percent of model scale) and rotation error (in degrees between the quaternions).} %Average rotation errors and position errors are provided. }%Two additional models are included in the average results (happy and eiffel) but excluded from the table for brevity as their results are similar to arma and rebel respectively.}
\label{tab:pose_est_results}
\end{table}

\begin{figure}
  \centering
   \includegraphics[width=1.0\linewidth]{supp_figures/noisy.pdf}
    \caption{\textbf{Noisy Pose Estimation} Dashed lines are averages for the method, while the black diamonds show the average for that method and model. Statistics for each method are listed with the \texttt{gear} model excluded.  Here Fuzzy Metaballs win in all statistical measures, typically by a factor of $\approx 2$. }
    \label{fig:noisy}
\end{figure}
%\begin{figure*}
%  \centering
%   \includegraphics[width=0.95\linewidth]{figures/example_grid_2row.pdf}
%    \caption{Fuzzy Metaballs from different numbers of components. Optimization can clean up model contours and depths. See ~\cref{sec:fitting}}
%    \label{fig:viz_results}
%\end{figure*}
%\begin{figure}[tb]
%  \centering
%   \includegraphics[width=1.0\linewidth]{figures/rms_prop_ex_small.pdf}
%    \caption{Optimizing Fuzzy Metaballs from a sphere to a shape. Losses are given for training frames and novel viewpoints, showing no significant difference. Qualitative results in \cref{fig:sill_results}.}
%    \label{fig:optimization}
%\end{figure}

==> qual_recon.tex <==
\begin{figure}[tbh]
     \centering
     \begin{subfigure}[t]{0.3\linewidth}
         \centering
         \includegraphics[trim={3cm 0 3cm 0},clip,width=\linewidth]{rebut_fig/plane_s_gt_when2.jpg}
         \caption{\textbf{Input} for Shape From Silhouette (SFS) task.}
         \label{fig:in_silh}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\linewidth}
         \centering
         \includegraphics[trim={2cm 0 2cm 0},clip,width=\linewidth]{rebut_fig/plane_pyt3d.jpg}
         \caption{\textbf{PyTorch3D Mesh} SFS of ShapeNet plane (100 min.)}
         \label{fig:pyt_plane}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\linewidth}
         \centering
         \includegraphics[trim={2cm 0 2cm 0},clip,width=\linewidth]{rebut_fig/yoga2_dss.jpg}
         \caption{\textbf{PyTorch3D Point Cloud} SFS of Yoga figurine (3 min.)}
         \label{fig:dss_yoga}
     \end{subfigure}
          \begin{subfigure}[t]{0.3\linewidth}
         \centering
         \includegraphics[trim={3cm 0 3cm 0},clip,width=\linewidth]{figures/plane_s_mine_when3.jpg}
         \caption{\textbf{Predicted Input} from converged FM}
         \label{fig:out_silh}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\linewidth}
         \centering
         \includegraphics[trim={2cm 0 2cm 0},clip,width=\linewidth]{figures/plane_mine_when_nocb4.jpg}
         \caption{\textbf{FM (Ours)} SFS of plane (45 sec.)}
         \label{fig:out_plane}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\linewidth}
         \centering
         \includegraphics[trim={2cm 0 2cm 0},clip,width=\linewidth]{figures/yoga_mine_eccv.jpg}
         \caption{\textbf{FM (Ours)} SFS of figurine (45 sec.)}
         \label{fig:out_yoga}
     \end{subfigure}
   \caption{\textbf{Qualitative baselines for shape-from-silhouette experiments} We used a ShapeNet airplane for the mesh baseline ~\cite{kato2017neural,liu2019soft,ravi2020pytorch3d} and the figurine of existing point cloud differentiable renderers~\cite{DSS_points}. Our best-effort mesh-based baseline result was incoherent and the point cloud baseline had spurious points. }
   \label{fig:rebutrecon}
\end{figure}

==> sil_fig.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/bunny_2k_fixed_1.jpg} }
     \end{subfigure}
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/bunny_2k_fixed_2.jpg} }
     \end{subfigure}
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/arma_2k_fixed_1.jpg} }
     \end{subfigure}
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/arma_2k_fixed_2.jpg} }
     \end{subfigure}
     \vfill
     
    \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/dragon_2k_fixed_1.jpg} }
     \end{subfigure}
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/dragon_2k_fixed_2.jpg} }
     \end{subfigure}
         \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/eiffel_tower_mini_fixed_1.jpg} }
     \end{subfigure}
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/eiffel_tower_mini_fixed_22.jpg} }
     \end{subfigure} 

    \vfill
       \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/happy_2k_fixed_15.jpg} }
     \end{subfigure}
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/happy_2k_fixed_3.jpg} }
     \end{subfigure}
            \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/lucy_2k_fixed_25.jpg} }
     \end{subfigure}
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/lucy_2k_fixed_29.jpg} }
     \end{subfigure}
     
     \vfill
            \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/rebelempire_fixed_1.jpg} }
     \end{subfigure}
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/rebelempire_fixed_26.jpg} }
     \end{subfigure}
                 \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/side_gear_fixed_14.jpg} }
     \end{subfigure}
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \fbox{ \centering \includegraphics[trim={0.75cm 0.75cm 0.75cm 0.75cm},clip,width=0.85\linewidth]{new_recon/side_gear_fixed_16.jpg} }
     \end{subfigure}
    \caption{\textbf{Shape from Silhouette (SFS)} reconstructions. On the left is a 40 component Fuzzy Metaball result and the right is the mesh ground-truth of about 2,500 faces, both colored by depth maps. See~\cref{sec:recon} for more details. }
    \label{fig:sill_results}
\end{figure}
